Telescope Concepts in Gamma-Ray Astronomy

This chapter outlines the general principles for the detection and characterisation of high-energy $\gamma$-ray photons in the energy range from MeV to GeV. Applications of these fundamental photon-matter interaction processes to the construction of instruments for $\gamma$-ray astronomy are described, including a short review of past and present realisations of telescopes. The constraints encountered in operating telescopes on high-altitude balloon and satellite platforms are described in the context of the strong instrumental background from cosmic rays as well as astrophysical sources. The basic telescope concepts start from the general collimator aperture in the MeV range over its improvements through coded-mask and Compton telescopes, to pair production telescopes in the GeV range. Other apertures as well as understanding the measurement principles of $\gamma$-ray astrophysics from simulations to calibrations are also provided.

==> 6_other_chapters.tex <==
To see the full Table of Contents of the Handbook see  \href{https://www.overleaf.com/project/5f7b1b1d2d65fe000101c619}{this link}.

\begin{center}
    \bf{Volume 1: X-ray Experimental Techniques and Missions}
\end{center}

\begin{center}
    \bf{From Section II: Detectors for X-ray Astrophysics}
\end{center}

\begin{itemize}

\item \textcolor{blue}{\bf Overview of Detectors for X-ray Astrophysics}
\begin{itemize}

\item Jan-Willem den Herder
\item Marco Feroci
\item Norbert Meidinger
\end{itemize}
\end{itemize}

\begin{center}
\bf{From Section III: X-ray Missions}
\end{center}

\begin{itemize}

\item \textcolor{blue}{\bf NuSTAR}
\begin{itemize}
\item Fiona Harrison
\end{itemize}

\item \textcolor{blue}{\bf Swift} 
\begin{itemize}
\item Lorella Angelini
\end{itemize}

\item \textcolor{blue}{\bf XMM-Newton} 
\begin{itemize}
\item Norbert Schartel
\item Maria Santos-Lleo
\end{itemize}

\end{itemize}
\begin{center}
    \bf{Volume 2: Gamma-ray Experimental Techniques, Observatories, and Missions}
\end{center}

\begin{itemize}
\item \textcolor{blue}{\bf History of Gamma-ray Astrophysics}
\begin{itemize}
\item Filippo Frontera
\item Andrea Santangelo
\end{itemize}
\end{itemize}

\begin{center}
    \bf{From Section IV: Optics and Detectors for Gamma-ray Astrophysics}
\end{center}

\begin{itemize}

\item \textcolor{blue}{\bf Telescope concepts in gamma-ray astronomy}
\begin{itemize}
\item The Three of Us
\end{itemize}

\item \textcolor{blue}{\bf Coded mask instruments}
\begin{itemize}
\item Andrea Goldwurm
\item Aleksandra Gros
\end{itemize}

\item \textcolor{blue}{\bf Temporal modulation aperture system}
\begin{itemize}
\item Pascal Saint-Hilaire
\item Gordon Hurford
\item Albert Shih
\item Brian Dennis
\end{itemize}

\item \textcolor{blue}{\bf Laue and Fresnel lenses}
\begin{itemize}
\item Hubert Halloin
\item Niels Lund
\item Gerald Skinner
\item Enrico Virgilli
\end{itemize}

\item \textcolor{blue}{\bf Compton telescopes} 
\begin{itemize}
\item Carolyn Kierans
\item Gottfried Kanbach
\item Tadayuki Takahashi
\end{itemize}


\item \textcolor{blue}{\bf Pair-creation telescopes} 
\begin{itemize}
\item David Thompson
\item Alexander Moiseev
\end{itemize}

\item \textcolor{blue}{\bf Orbits and background of gamma-ray space instruments}
\begin{itemize}
\item Vincent Tatischeff
\item Pietro Ubertini
\item Tsunefumi Mizuno
\end{itemize}


\item \textcolor{blue}{\bf Germanium detectors for gamma-ray astronomy} 
\begin{itemize}
\item Jean-Pierre Roques
\end{itemize}

\item \textcolor{blue}{\bf Silicon detectors for gamma-ray astronomy} 
\begin{itemize}
\item Regina Caputo
\end{itemize}

\item \textcolor{blue}{\bf CdTe and CZT detectors for gamma-ray astronomy} 
\begin{itemize}
\item Ezio Caroli
\end{itemize}

\item \textcolor{blue}{\bf Scintillators for gamma-ray astronomy}
\begin{itemize}
\item Anatoly Iyudin
\item Claudio Labanti
\item Oliver Roberts
\end{itemize}

\item \textcolor{blue}{\bf Photodetectors for gamma-ray astronomy} 
\begin{itemize}
\item Elisabetta Bissaldi
\item Carlo Fiorini
\item Alexey Uliyanov
\end{itemize}

\item \textcolor{blue}{\bf Time projection chambers for gamma-ray astronomy} 
\begin{itemize}
\item Denis Bernard
\item Stanley Hunter
\item Toru Tanimori
\end{itemize}

\item \textcolor{blue}{\bf Readout electronics for gamma-ray astronomy}
\begin{itemize}
\item Marco Carminati
\item Carlo Fiorini
\end{itemize}

\item  \textcolor{blue}{\bf Design of gamma-ray polarimeters} 
\begin{itemize}
\item Denis Bernard
\item Tanmoy Chattopadhyay
\item Fabian Kislat
\item Nicolas Produit
\end{itemize}

\item \textcolor{blue}{\bf CubeSats for gamma-ray astronomy} 
\begin{itemize}
\item Peter Bloser
\item Fabrizio Fiore
\item Sheila McBreen
\item Jeremy Perkins
\end{itemize}

\item \textcolor{blue}{\bf Detector and mission design simulations} 
\begin{itemize}
\item Eric Charles
\item Henrike Fleischhack
\item Clio Sleator
\end{itemize}
\end{itemize}

\begin{center}
    \bf{From Section V: Space-based Gamma-ray Observatories}
\end{center}

\begin{itemize}

\item \textcolor{blue}{\bf The Compton Gamma-ray Observatory} 
\begin{itemize}
\item Author(s) TBC
\end{itemize}

\item \textcolor{blue}{\bf The COMPTEL instrument on the CGRO mission} 
\begin{itemize}
\item James Ryan
\item Volker Sch\"{o}nfelder
\end{itemize}

\item \textcolor{blue}{\bf The INTErnational Gamma-Ray Astrophysics Laboratory (INTEGRAL)} 
\begin{itemize}
\item Peter Kretschmar
\item Erik Kuulkers
\item Philippe Laurent
\end{itemize}

\item \textcolor{blue}{\bf The AGILE mission} 
\begin{itemize}
\item Francesco Longo
\end{itemize}

\item \textcolor{blue}{\bf The Fermi Gamma-ray Space Telescope mission} 
\begin{itemize}
\item David J. Thompson
\item Colleen Wilson-Hodge
\end{itemize}

\item \textcolor{blue}{\bf The Large Area Telescope on the Fermi mission} 
\begin{itemize}
\item Riccardo Rando
\end{itemize}

\item \textcolor{blue}{\bf Future prospects for gamma-ray telescopes} 
\begin{itemize}
\item Author(s) TBC
\end{itemize}
\end{itemize}

\begin{center}
    \bf{From Section VI: Ground-based Gamma-ray Observatories}
\end{center}

\begin{itemize}

\item \textcolor{blue}{\bf Introduction to ground-based Gamma-ray astrophysics} 
\begin{itemize}
\item Alberto Carramiñana
\item Emma de Ona Wilhelmi
\item Andrew Taylor
\end{itemize}

\item \textcolor{blue}{\bf How to detect Gamma-rays from ground: an introduction to the detection concepts} 
\begin{itemize}
\item Manel Errando
\item Takayuki Saito
\end{itemize}

\item \textcolor{blue}{\bf The development of ground-based Gamma-ray astronomy: a historical overview of the pioneering experiments}
\begin{itemize}
\item Razmik Mirzoyan
\end{itemize}

\end{itemize}

